MCA-based Rule Mining Enables Interpretable Inference in Clinical Psychiatry

Development of interpretable machine learning models for clinical healthcare applications has the potential of changing the way we understand, treat, and ultimately cure, diseases and disorders in many areas of medicine. These models can serve not only as sources of predictions and estimates, but also as discovery tools for clinicians and researchers to reveal new knowledge from the data. High dimensionality of patient information (e.g., phenotype, genotype, and medical history), lack of objective measurements, and the heterogeneity in patient populations often create significant challenges in developing interpretable machine learning models for clinical psychiatry in practice. In this paper we take a step towards the development of such interpretable models. First, by developing a novel categorical rule mining method based on Multivariate Correspondence Analysis (MCA) capable of handling datasets with large numbers of features, and second, by applying this method to build transdiagnostic Bayesian Rule List models to screen for psychiatric disorders using the Consortium for Neuropsychiatric Phenomics dataset. We show that our method is not only at least 100 times faster than state-of-the-art rule mining techniques for datasets with 50 features, but also provides interpretability and comparable prediction accuracy across several benchmark datasets.

==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgements}
\label{sec:acknowledgements}

\todo{Placeholder}.


==> sections/reviews.tex <==
\section{Reviewer Comments \todo{temporary section}}

\subsection{Review 1}

\paragraph{Overall evaluation:} 2 (accept)

In the paper the authors propose MCA-miner -- a new algorithm for generating decision rules that employs multivariate correspondence analysis (MCA) to evaluate candidate rules.
The algorithm is integrated with the MCMC search algorithm aimed at constructing Bayesian rule lists (BRLs).
MCA-miner is much more efficient (in terms of computation time) than traditionally considered approaches (e.g., FP-Growth) and scales better with the number of attributes/categorical values.
The authors also present a parallel implementation of the MCMC algorithm that leads to further time savings.
Finally, in computational experiments the authors first apply their proposal (BRL with MCA-miner) to a several benchmark data sets, and then to a CNP psychiatric data set (with 578 attributes and 1350 categorical values).
For the latter data set they present models obtained for two different decision problems and discuss their performance and interpretability.

The paper is very well written, fits the scope of the workshop and the results show advantages of MCA-miner as well as usefulness of BRLs for a specific clinical application.
There are still some minor issues (listed below) the authors should address in the final version of the text.

\begin{enumerate}
\item There are different aspects of interpretability as discussed in~\cite{lipton2018mythos} and the authors should better explain what type of interpretability their approach supports.

  \review{%
    Add citation and comment related to Lipton's article.
  }
  \todo{done}

\item In the Abstract the authors refer to ``transdiagnostic model.''
  It would be informative to explain how to understand this is the context of the described study.
  Does it mean multi-class?

  \review{%
    Missing explanation between multi-class and transdiagnostic.
    Right now we are multi-class, but interpretability enables us to understand transdiagnosis.
  }
  \todo{done}

\item In Section~1 the authors refer to ``predictable models.''
  Again, it is not clear what the authors mean by this -- a brief explanation would be helpful.

  \review{%
    Typo, should be ``predictive''.
  }
  \todo{done}

\item Several times in the text the authors mention ``statistical significance'' (e.g., in the context of Table~2).
  However, no information about such tests or their results is provided.
  The authors should revise the text to remove this confusion.

  \review{%
    We should use ``effect size'' instead, and cite Cohen $\kappa$ as our tool of choice.
  }
  \todo{done}

\item It is not clear what data set was used to build a binary classifier from the CNP data set.
  Did the authors balance the distribution of classes (Patients vs.\ HC).
  If yes, how many examples were considered in each class?

  \review{%
    Question for Clark, simply add explanation in Section~5.3.
  }
  \todo{done}
\end{enumerate}


\subsection{Review 2}

\paragraph{Overall evaluation:} 2 (accept)

The authors propose a two-step approach to learning interpretable predictive models in clinical psychiatry.
The authors use a Multiple Correspondence Analysis (MCA) miner to extract rules used to construct a Bayesian Rule List (BRL) model to screen for neuropsychiatric disorders.
The work is innovative and has been shown to significantly improve over existing state-of-the-art approaches.
It also addresses the very important issue of interpretability, contributing to the field of explainable AI (XAI).
The work is very well motivated and the experimental setup and results are convincing.
I would have appreciated more discussion about the clinical application of the work (i.e., CDSS) and future directions for research.

\review{%
  Do we want to talk about consequences of our results in recruitment for clinical trials?
  Add a comment about future research directions? \todo{done}

  Cite CDSS and describe our approach in the context of the work since 1972. \todo{done}
}

Minor comment about presentation.
There are several figures that appear much later in the text (several pages) from where they are first referenced.
This makes it a little difficult to follow the text and look at the figures.
Also, the last two pages are mostly figures and tables with text interjected.
It would help paper readability to improve the positioning of the figures and tables and improve the text layout.

\review{%
  Shuffle figures so they appear closer to the relevant text.
}
\todo{done}
